Breaking 3-Factor Approximation for Correlation Clustering in Polylogarithmic Rounds

In this paper, we study parallel algorithms for the correlation clustering problem, where every pair of two different entities is labeled with similar or dissimilar. The goal is to partition the entities into clusters to minimize the number of disagreements with the labels. Currently, all efficient parallel algorithms have an approximation ratio of at least 3. In comparison with the $1.994+\epsilon$ ratio achieved by polynomial-time sequential algorithms [CLN22], a significant gap exists. We propose the first poly-logarithmic depth parallel algorithm that achieves a better approximation ratio than 3. Specifically, our algorithm computes a $(2.4+\epsilon)$-approximate solution and uses $\tilde{O}(m^{1.5})$ work. Additionally, it can be translated into a $\tilde{O}(m^{1.5})$-time sequential algorithm and a poly-logarithmic rounds sublinear-memory MPC algorithm with $\tilde{O}(m^{1.5})$ total memory. Our approach is inspired by Awerbuch, Khandekar, and Rao's [AKR12] length-constrained multi-commodity flow algorithm, where we develop an efficient parallel algorithm to solve a truncated correlation clustering linear program of Charikar, Guruswami, and Wirth [CGW05]. Then we show the solution of the truncated linear program can be rounded with a factor of at most 2.4 loss by using the framework of [CMSY15]. Such a rounding framework can then be implemented using parallel pivot-based approaches.

==> overview.tex <==
We start from precisely defining the linear programs we will be working on.

\paragraph{Primal (Triangle Inequality View).}
\begin{equation}
\begin{aligned}
    \text{minimize }\ \  & \sum_{(u, v)\in E^+} x_{uv} + \sum_{(u, v)\in E^-} (1-x_{uv}) \\
    \text{subject to }\ \  & \begin{aligned}[t] 
    & x_{uw} + x_{wv} \ge x_{uv} && \ \ \forall u, v, w\in V\\
    & x_{uu} = 0 && \ \ \forall u\in V\\
    & x_{uv} \in [0, 1] && \ \ \forall (u, v)\in E
    \end{aligned} 
\end{aligned}\tag{P1}
\end{equation}

\paragraph{Primal (Shortest Path View).}
\begin{equation}
\begin{aligned}
    \text{minimize }\ \  & \sum_{(u, v)\in E^+} x_{uv} + \sum_{(u, v)\in E^-} z_{uv} \\
    \text{subject to }\ \  & \begin{aligned}[t]
    & z_{uv} + \sum_{e\in P_{uv}} x_e \ge 1 && \ \ \forall (u, v)\in E^-\text{ and $uv$-path } P_{uv}\subseteq G^+\\
    & x_{e} \ge 0, z_{f}\ge 0 && \ \ \forall e\in E^+, f\in E^-
    \end{aligned} 
\end{aligned}\tag{\PRIMAL}
\end{equation}

\paragraph{Almost Primal ($L$-hop-limited Shortest Path View).}
\begin{equation}
\begin{aligned}
    \text{minimize }\ \  & \sum_{(u, v)\in E^+} x_{uv} + \sum_{(u, v)\in E^-} z_{uv} \\
    \text{subject to }\ \  & \begin{aligned}[t]
    & z_{uv} + \sum_{e\in P_{uv}} x_e \ge 1 && \ \ \begin{aligned}[t]
    \forall (u, v)\in E^-\text{ and $uv$-path } P_{uv}\subseteq G^+ \\
    \text{ such that } |P_{uv}|\le L
    \end{aligned}\\
    & x_{e} \ge 0, z_{f}\ge 0 && \ \ \forall e\in E^+, f\in E^-
    \end{aligned} 
\end{aligned}\tag{\PRIMALELL}
\end{equation}

\paragraph{Two-Hop Primal ($L=2$).}
\begin{equation}
\begin{aligned}
    \text{minimize }\ \  & \sum_{(u, v)\in E^+} x_{uv} + \sum_{(u, v)\in E^-} z_{uv} \\
    \text{subject to }\ \  & \begin{aligned}[t]
    & z_{uv} + x_{uw} + x_{wv} \ge 1 && \ \ 
    \forall (u, v)\in E^-\text{ and } (u, w), (w, v)\in E^+ \\
    & x_{e} \ge 0, x_{e'}\ge 0 && \ \ \forall e\in E^+,  e'\in E^-
    \end{aligned} 
\end{aligned}\tag{$\PRIMAL^{(2)}$}
\end{equation}


\paragraph{Two-Hop Dual.} Let $\PTwo$ be the collection of length-two paths $(u, w, v)$ such that $(u, w), (w, v)\in E^+$ and $(u, v)\in E^-$.
\begin{equation}
\begin{aligned}
    \text{maximize }\ \  & \sum_{(u, w, v)\in \PTwo} y_{(u, w, v)} \\
    \text{subject to }\ \  & \begin{aligned}[t]
    & \sum_{w: (u, w, v)\in \PTwo} y_{(u, w, v)} \le 1 && \ \ 
    \forall (u, v)\in E^- \\
    & \sum_{v': (u, w, v')\in \PTwo} y_{(u, w, v')} + \sum_{u': (u', w, u)\in\PTwo} y_{(u', w, u)}  \le 1 && \ \ \forall (u, w)\in E^+\\
    & y_{(u, w, v)}\ge 0 && \ \ \forall (u, w, v)\in \PTwo
    \end{aligned} 
\end{aligned}\tag{$\DUALTWO$}
\end{equation}

\subsection{Outline of the Main Algorithm}

Our algorithm starts with computing an $(1+\epsilon)$-approximate solution 
$\{x_{ab}, z_{uv}\}$ to $\PRIMAL^{(2)}$, via a variant to the \emph{steepest descent framework} originated by Awerbuch, Khandekar, and Rao~[].
The steepest descent framework actually solves for an $(1+\epsilon)$-approximate solution $\{y_{(u, w, v)}\}$ to $\DUALTWO$, but as a by-product the algorithm actually obtains approximate solutions to $\PRIMAL^{(2)}$ as well.
Then, we apply an 2.5-approximate rounding algorithm provided by Ailon, Charikar, and Newman~[].
Although the rounding algorithm is almost identical, the analysis are slightly different.
In particular, the optimal solution of $\PRIMAL^{(2)}$ may not satisfy the triangle inequality anymore.
However, our crucial observation shows that the rounding algorithm still correctly outputs a $2.5$-approximate solution.

